An Artificial Neural Network-Based Model Predictive Control for Three-phase Flying Capacitor Multi-Level Inverter

Model predictive control (MPC) has been used widely in power electronics due to its simple concept, fast dynamic response, and good reference tracking. However, it suffers from parametric uncertainties, since it directly relies on the mathematical model of the system to predict the optimal switching states to be used at the next sampling time. As a result, uncertain parameters lead to an ill-designed MPC. Thus, this paper offers a model-free control strategy on the basis of artificial neural networks (ANNs), for mitigating the effects of parameter mismatching while having a little negative impact on the inverter's performance. This method includes two related stages. First, MPC is used as an expert to control the studied converter in order to provide a dataset, while, in the second stage, the obtained dataset is utilized to train the proposed ANN. The case study herein is based on a four-level three-cell flying capacitor inverter. In this study, MATLAB/Simulink is used to simulate the performance of the proposed method, taking into account various operating conditions. Afterward, the simulation results are reported in comparison with the conventional MPC scheme, demonstrating the superior performance of the proposed control strategy in terms of robustness against parameters mismatch and low total harmonic distortion (THD), especially when changes occur in the system parameters, compared to the conventional MPC. Furthermore, the experimental validation of the proposed method is provided based on the Hardware-in-the-Loop (HIL) simulation using the C2000TM-microcontroller-LaunchPadXL TMS320F28379D kit, demonstrating the applicability of the ANN-based control strategy to be implemented on a DSP controller.

==> ANN2.tex <==
%\documentclass[border=0.125cm]{standalone}
%\usepackage{tikz}
%\usetikzlibrary{positioning}
%\begin{document}

\tikzset{%
  every neuron/.style={
    circle,
    draw,
    very thick,
    
    minimum size=1cm,
  },
  neuron missing/.style={
    draw=none, 
    scale=4,
    text height=0.333cm,
    execute at begin node=\color{black}$\vdots$
  },
}

\begin{tikzpicture}[x=1.5cm, y=1.7cm, >=stealth]
%\tikzstyle{input}=[neuron, fill=green!50];
%\tikzstyle{output}=[neuron, fill=red!50];
%\tikzstyle{hidden}=[neuron, fill=blue!50];

\foreach \m/\l [count=\y] in {1,2,3,missing,4}
  \node [ every neuron/.try, neuron \m/.try,red] (input-\m) at (0,2.5-\y) {};

\foreach \m [count=\y] in {1,2,missing,3}
  \node [every neuron/.try, neuron \m/.try, blue] (hidden-\m) at (1.5,2-\y*1) {};

\foreach \m [count=\y] in {1}
  \node [every neuron/.try, neuron \m/.try,green] (output-\m) at (3,0.8-\y) {};

\foreach \l [count=\i] in {1,2,3,n}
  \draw [very thick,<-,red] (input-\i) -- ++(-1,0)
    node [above, midway,black] {$I_\l$};

\foreach \l [count=\i] in {1,2,n}
  \node [above] at (hidden-\i.north) {$H_\l$};

\foreach \l [count=\i] in {1}
  \draw [very thick,->,orange] (output-\i) -- ++(1,0)
    node [above,midway,black] {Output};

\foreach \i in {1,...,4}
  \foreach \j in {1,...,3}
    \draw [very thick,->,blue] (input-\i) -- (hidden-\j);

\foreach \i in {1,...,3}
  \foreach \j in {1}
    \draw [very thick,->,green] (hidden-\i) -- (output-\j);


\foreach \l [count=\x from 0] in {Input, Hidden, Output}
\node [align=center, above] at (\x*1.5,2) {\l \\ layer};


\end{tikzpicture}

%\end{document}

==> P2.tex <==
%\documentclass{article}

%\usepackage{tikz}
%\usetikzlibrary{calc}
%\usepackage{graphicx}

%\begin{document}
    %\centering
    \begin{tikzpicture}
        
        \begin{scope}[xshift=4.5cm]
        \node[minimum width=3cm,minimum height=2cm,inner sep=0pt,draw,fill={rgb:pink,10},rounded corners] (textA) {\textbf{MPC}};
        \end{scope}
        
        \begin{scope}[xshift=10.5cm]
        \node[minimum width=6cm,minimum height=6cm,inner sep=0pt,draw,color = red!40, fill = yellow!10,rounded corners] (imageB) {\includegraphics[width=5cm]{FIG/K1.pdf}};
        \end{scope}
        
        
         \begin{scope}[xshift=17.5cm]
           \node[minimum width=6cm,minimum height=6cm,inner sep=0pt,draw,color = blue!40, fill = yellow!10,rounded corners] (imageC) {\includegraphics[width=5cm]{FIG/3phase.pdf}};
  

        \end{scope}
        
        %finally, add arrows
      
        \draw[very thick,->,>=stealth] ($(textA.east)+(0.2,0)$) -- ($(imageB.west)+(-0.2,0)$) node [text width=2.5cm,midway,above,align=center,font=\tiny] {training Dataset};
        
         \draw[very thick,->,>=stealth] ($(imageB.east)+(0.2,0)$) -- ($(imageC.west)+(-0.2,0)$) node [text width=2.5cm,midway,above,align=center,font=\tiny] {$S_{opt}$};
    \end{tikzpicture}
%\end{document}
